Proactive Assistant Dialogue Generation from Streaming Egocentric Videos

Recent advances in conversational AI have been substantial, but developing real-time systems for perceptual task guidance remains challenging. These systems must provide interactive, proactive assistance based on streaming visual inputs, yet their development is constrained by the costly and labor-intensive process of data collection and system evaluation. To address these limitations, we present a comprehensive framework with three key contributions. First, we introduce a novel data curation pipeline that synthesizes dialogues from annotated egocentric videos, resulting in \dataset, a large-scale synthetic dialogue dataset spanning multiple domains. Second, we develop a suite of automatic evaluation metrics, validated through extensive human studies. Third, we propose an end-to-end model that processes streaming video inputs to generate contextually appropriate responses, incorporating novel techniques for handling data imbalance and long-duration videos. This work lays the foundation for developing real-time, proactive AI assistants capable of guiding users through diverse tasks. Project page: https://pro-assist.github.io/

==> figures/metrics_vs_attribute.tex <==

\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{imgs/duration.pdf}
    \caption{Overall score v.s. task duration in minutes.}
    \label{fig:subfig1}
\end{subfigure}
~
\begin{subfigure}[b]{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{imgs/proactive_rate.pdf}
    \caption{Overall score v.s. the ratio of proactive response in reference.\vspace{-5pt}}
    \label{fig:subfig2}
\end{subfigure}
\caption{Correlation between overall score and task properties.\vspace{-15pt}}
\label{fig:vs_attribute}
\end{figure}

==> figures/progress_summary.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{imgs/progress_summary.pdf}
    \vspace{-5pt}
    \caption{Illustration of iterative progress summary. The model is prompted to generate a summary of progress upon approaching its maximum context length. Generation then restarts with an initial system prompt incorporated with the generated progress summary.\vspace{-10pt}}
    \label{fig:progress_summarization}
\end{figure}

==> tables/offline_vs_online.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|cc|cc}
    \toprule
     \multirow{2}{*}{Context}& \multicolumn{2}{c|}{Action Narration}  & \multicolumn{2}{c}{Dialogue Generation} \\
    & METEOR &   BLEU &   METEOR & BLEU \\
    \midrule
      GT  & 36.35 & 48.78 & 21.37 & 23.17 \\
 Self & 21.67 & 13.81 & 19.94 & 16.47 \\
 % I=1 & GT  & 36.35 & 48.78 & 21.37 & 23.17 \\
 % I=1  & Self & 21.67 & 13.81 & 19.94 & 16.47 \\
 % \hline
 % I=5 & GT   & 35.57 & 47.23 & 20.86 & 21.92 \\
 % I=5   & Self           & 21.68 & 13.77 & 19.05 & 15.36 \\
 %  \hline
 % I=10 & GT & 35.47 & 46.44 & 21.24 & 21.98 \\
 % I=10  & Self          & 22.36 & 14.66 & 18.80 & 14.99 \\
    \bottomrule
    \end{tabular}
    \caption{Comparison of the dialogue generation quality between online evaluation with self-generated context with offline evaluation with ground-truth context.}
    \label{tab:offline-vs-online}
\end{table}
